Multirate Linearly-Implicit GARK Schemes

Many complex applications require the solution of initial-value problems where some components change fast, while others vary slowly. Multirate schemes apply different step sizes to resolve different components of the system, according to their dynamics, in order to achieve increased computational efficiency. The stiff components of the system, fast or slow, are best discretized with implicit base methods in order to ensure numerical stability. To this end, linearly implicit methods are particularly attractive as they solve only linear systems of equations at each step. This paper develops the Multirate GARK-ROS/ROW (MR-GARK-ROS/ROW) framework for linearly-implicit multirate time integration. The order conditions theory considers both exact and approximative Jacobians. The effectiveness of implicit multirate methods depends on the coupling between the slow and fast computations; an array of efficient coupling strategies and the resulting numerical schemes are analyzed. Multirate infinitesimal step linearly-implicit methods, that allow arbitrarily small micro-steps and offer extreme computational flexibility, are constructed. The new unifying framework includes existing multirate Rosenbrock(-W) methods as particular cases, and opens the possibility to develop new classes of highly effective linearly implicit multirate integrators.

==> bookfile.tex <==




For multirate GARK-ROW schemes we get for order 1
%
\begin{subequations}
\label{eqn:multirate-GARK-ROW-order3-conditions}
\begin{eqnarray}
&& \mathbf{b}^{\{\slow\}\,T} \, \one = 1,  \\
                         && \mathbf{b}^{\{\fast\}\,T} \, \one = 1, 
                         \end{eqnarray}
\end{subequations}                         
for order 2
\begin{subequations}
\begin{eqnarray}
&&
\mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\slow\}} \, \boldsymbol{1} = \frac{1}{2}, \\
&&\mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\fast,1\}} \, \boldsymbol{1} = \frac{M}{2},\\
&&\mathbf{b}^{\{\fast\}\,T} \, 
 \boldsymbol{\alpha}^{\{\fast,\fast\}} 
 \, \boldsymbol{1} = \frac{1}{2}, \\
&&\mathbf{b}^{\{\fast\}\,T} \, \left( \sum_{\lambda=1}^M \boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}} \right) \, \boldsymbol{1} = \frac{M}{2},\\
&&
\mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\slow\}} \, \boldsymbol{1} = 0, \\
&&\mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\fast,1\}} \, \boldsymbol{1} = 0,\\
&&\mathbf{b}^{\{\fast\}\,T} \, \left( \sum_{\lambda=1}^M \boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}} \right) \, \boldsymbol{1} = 0,\\
&&\mathbf{b}^{\{\fast\}\,T} \, \left( \sum_{\lambda=1}^M \boldsymbol{\gamma}^{\{\fast,\slow,\lambda\}} \right) \, \boldsymbol{1} = 0,
\end{eqnarray}
and for order 3;
\begin{eqnarray}
 &&
%\begin{cases}
\mathbf{b}^{\{\slow\}\,T} \, \bigl( (\boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1})\times (\boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1}) \bigr) = \frac{1}{3}, \\
&& \mathbf{b}^{\{\slow\}\,T} \, \bigl( (\boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1})\times (\boldsymbol{\alpha}^{\{\slow,\fast,1\}}\,\mathbf{1}) \bigr) = \frac{M}{3}, \\
&& \mathbf{b}^{\{\slow\}\,T} \, \bigl( (\boldsymbol{\alpha}^{\{\slow,\fast,1\}}\,\mathbf{1})\times (\boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1}) \bigr) = \frac{M}{3}, \\
&& \mathbf{b}^{\{\slow\}\,T} \, \bigl( (\boldsymbol{\alpha}^{\{\slow,\fast,1\}}\,\mathbf{1})\times (\boldsymbol{\alpha}^{\{\slow,\fast,1\}}\,\mathbf{1}) \bigr) = \frac{M^2}{3}, \\
&&
%\mathbf{b}^{\{\fast\}\,T} \, \bigl( (\boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1})\times (\boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1}) 
%- \frac{M-1}{M} \sum_{\lambda=1}^M  \boldsymbol{\gamma}^{\{\fast,\fast,\lambda \}}\,\mathbf{1}
%\bigr) = \frac{1}{3}, \\
\mathbf{b}^{\{\fast\}\,T} \, \bigl( (\boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1})\times (\boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1}) 
= \frac{1}{3}, \\
&& \mathbf{b}^{\{\fast\}\,T} \,  \sum_{\lambda=1}^M  
\Bigl( 
\left( \boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1}
\right) \times 
\left( \boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}} \,\mathbf{1}
 \right)
+ (\lambda-1) \boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}}
\,\mathbf{1}
\Bigr)  
  =  \frac{M^2}{3}, \\
%&& \mathbf{b}^{\{\fast\}\,T} \, \Bigl( \sum_{\lambda=1}^M  \left( \boldsymbol{\alpha}^{\{\fast,\fast\}}\,
% \boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}} 
%+ (\lambda-1) \boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}} \right)
%\Bigr)  \,\mathbf{1}  =  \frac{M^2}{3}, \\
%&& \mathbf{b}^{\{\fast\}\,T} \, \Bigl( \sum_{\lambda=1}^M  \left( \boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}}\,
% \boldsymbol{\alpha}^{\{\fast,\fast\}} 
%+ (\lambda-1) \boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}} \right)
%\Bigr)  \,\mathbf{1}  =  \frac{M^2}{3}, \\
&& \mathbf{b}^{\{\fast\}\,T} \,  \sum_{\lambda=1}^M  
\Bigl( 
\left( \boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}}\,\mathbf{1}
\right) \times 
\left( \boldsymbol{\alpha}^{\{\fast,\fast\}} \,\mathbf{1}
 \right)
+ (\lambda-1) \boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}}
\,\mathbf{1}
\Bigr)  
  =  \frac{M^2}{3}
 \\
&& \mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M \bigl( (\boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}}\,\mathbf{1})\times (\boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}}\,\mathbf{1}) \bigr) = \frac{M}{3}, \\
  \end{eqnarray}
  \end{subequations}
  
\begin{subequations}
  \begin{eqnarray}
&&  \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\slow\}}\, \boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1} = \frac{1}{6} \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\slow\}}\, \boldsymbol{\alpha}^{\{\slow,\fast,1\}}\,\mathbf{1} = \frac{M}{6} \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\fast,1\}}\, \boldsymbol{\alpha}^{\{\fast,\slow,1\}}\,\mathbf{1} = \frac{M}{6} \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\fast,1\}}\, \boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1} = \frac{M^2}{6} \\
&&  \mathbf{b}^{\{\fast\}\,T} \, \boldsymbol{\alpha}^{\{\fast,\fast\}}\, \boldsymbol{\alpha}^{\{\fast,\fast,\}}\,\mathbf{1} = \frac{1}{6} \\
&& \mathbf{b}^{\{\fast\}\,T} \, \left(
\sum_{\lambda=1}^M \boldsymbol{\alpha}^{\{\fast,\fast\}}\, \boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}} +
 \sum_{\lambda=1}^{M-1} (M-\lambda) \boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}}
\right) \,\mathbf{1} = \frac{M^2}{6} \\
&& \mathbf{b}^{\{\fast\}\,T} \, 
\left( \sum_{\lambda=1}^M \boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}}
\right) \, 
 \boldsymbol{\alpha}^{\{\slow,\fast,1\}}
 \,\mathbf{1} = \frac{M^2}{6} \\
&& \mathbf{b}^{\{\fast\}\,T} \, 
\left( \sum_{\lambda=1}^M \boldsymbol{\alpha}^{\{\fast,\slow,\lambda \}}
\right) \, \boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1} = \frac{M}{6}
\end{eqnarray}
\end{subequations}
%


\begin{subequations}
\begin{eqnarray}
&&
%\begin{cases}
 \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\slow\}}\, \boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1} = 0 \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\slow\}}\, \boldsymbol{\alpha}^{\{\slow,\fast,1\}}\,\mathbf{1} = 0 \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\fast,1\}}\, \boldsymbol{\alpha}^{\{\fast,\slow,1\}}\,\mathbf{1} = 0 \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\fast,1\}}\, \boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1} = 0 \\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}}
\, 
\boldsymbol{\alpha}^{\{\fast,\fast\}} %+ (\lambda-1) ]
\,\mathbf{1}
 = 0, 
\\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}}
\, 
\boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}}\,\mathbf{1}
 = 0, 
\\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\gamma}^{\{\fast,\slow,\lambda\}}
\, 
\boldsymbol{\alpha}^{\{\slow,\fast,1\}}\,\mathbf{1}
 = 0, 
\\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\gamma}^{\{\fast,\slow,\lambda\}}
\, 
\boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1}
 = 0, 
\end{eqnarray}
\end{subequations}



\begin{subequations}
\begin{eqnarray}
&&  \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\slow\}}\, \boldsymbol{\gamma}^{\{\slow,\slow\}}\,\mathbf{1} = 0 \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\slow\}}\, \boldsymbol{\gamma}^{\{\slow,\fast,1\}}\,\mathbf{1} = 0 \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\fast,1\}}\, \boldsymbol{\gamma}^{\{\fast,\slow,1\}}\,\mathbf{1} = 0 \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\fast,1\}}\, \boldsymbol{\gamma}^{\{\fast,\fast,1\}}\,\mathbf{1} = 0 \\
 &&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M  \left[
\boldsymbol{\alpha}^{\{\fast,\fast\}} \, 
\boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}}
+ (M-\lambda) \boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}}
\right]
\,\mathbf{1}
 = 0, 
\\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M  \left[
\boldsymbol{\alpha}^{\{\fast,\fast\}} \, 
\boldsymbol{\gamma}^{\{\fast,\slow,1\}}
+ (M-\lambda) \boldsymbol{\gamma}^{\{\fast,\slow,1\}}
\right]
\,\mathbf{1}
 = 0, 
\\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}}
\, 
\boldsymbol{\gamma}^{\{\slow,\fast,1\}}\,\mathbf{1}
 = 0, 
\\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}}
\, 
\boldsymbol{\gamma}^{\{\slow,\slow\}}\,\mathbf{1}
 = 0, 
\end{eqnarray}
\end{subequations}



\begin{subequations}
\begin{eqnarray}
&&  \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\slow\}}\, \boldsymbol{\gamma}^{\{\slow,\slow\}}\,\mathbf{1} = 0 \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\slow\}}\, \boldsymbol{\gamma}^{\{\slow,\fast,1\}}\,\mathbf{1} = 0 \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\fast,1\}}\, \boldsymbol{\gamma}^{\{\fast,\slow,1\}}\,\mathbf{1} = 0 \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\fast,1\}}\, \boldsymbol{\gamma}^{\{\fast,\fast,1\}}\,\mathbf{1} = 0 \\
 &&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}}
\, 
\boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}}\,\mathbf{1}
 = 0, 
\\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}}
\, 
\boldsymbol{\gamma}^{\{\fast,\slow,\lambda\}}\,\mathbf{1}
 = 0, 
\\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\gamma}^{\{\fast,\slow,\lambda\}}
\, 
\boldsymbol{\gamma}^{\{\slow,\fast,1\}}\,\mathbf{1}
 = 0, 
\\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\gamma}^{\{\fast,\slow,\lambda\}}
\, 
\boldsymbol{\gamma}^{\{\slow,\slow\}}\,\mathbf{1}
 = 0, 
\end{eqnarray}
\end{subequations}














The number of order conditions can be significantly reduced, if we use internally consistent schemes: the order one conditions
\begin{subequations}
\label{eqn:multirate-GARK-ROW-order3-conditions}
\begin{eqnarray}
&& \mathbf{b}^{\{\slow\}\,T} \, \one = 1,  \\
                         && \mathbf{b}^{\{\fast\}\,T} \, \one = 1, 
                         \end{eqnarray}
\end{subequations}    
remain, the order 2 conditions reduce to
\begin{subequations}
\begin{eqnarray}
&&
\mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\slow\}} \, \boldsymbol{1} = \frac{1}{2}, \\
&&\mathbf{b}^{\{\fast\}\,T} \, 
 \boldsymbol{\alpha}^{\{\fast,\fast\}} 
 \, \boldsymbol{1} = \frac{1}{2}, \\
&&
\mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\slow\}} \, \boldsymbol{1} = 0, \\
&&\mathbf{b}^{\{\fast\}\,T} \, \left( \sum_{\lambda=1}^M \boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}} \right) \, \boldsymbol{1} = 0,
\end{eqnarray}
and for order 3 we get;
\begin{eqnarray}
 &&
%\begin{cases}
\mathbf{b}^{\{\slow\}\,T} \, \bigl( (\boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1})\times (\boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1}) \bigr) = \frac{1}{3}, \\
&&
\mathbf{b}^{\{\fast\}\,T} \, \bigl( (\boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1})\times (\boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1}) 
= \frac{1}{3}
  \end{eqnarray}
  \end{subequations}
  
\begin{subequations}
  \begin{eqnarray}
&&  \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\slow\}}\, \boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1} = \frac{1}{6} \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\fast,1\}}\, \boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1} = \frac{M^2}{6} \\
&&  \mathbf{b}^{\{\fast\}\,T} \, \boldsymbol{\alpha}^{\{\fast,\fast\}}\, \boldsymbol{\alpha}^{\{\fast,\fast,\}}\,\mathbf{1} = \frac{1}{6} \\
&& \mathbf{b}^{\{\fast\}\,T} \, 
\left( \sum_{\lambda=1}^M \boldsymbol{\alpha}^{\{\fast,\slow,\lambda \}}
\right) \, \boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1} = \frac{M}{6}
\end{eqnarray}
\end{subequations}
%


\begin{subequations}
\begin{eqnarray}
&&
%\begin{cases}
 \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\slow\}}\, \boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1} = 0 \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\fast,1\}}\, \boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1} = 0 \\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}}
\, 
\boldsymbol{\alpha}^{\{\fast,\fast\}} %+ (\lambda-1) ]
\,\mathbf{1}
 = 0, 
\\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\gamma}^{\{\fast,\slow,\lambda\}}
\, 
\boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1}
 = 0, 
\end{eqnarray}
\end{subequations}



\begin{subequations}
\begin{eqnarray}
&&  \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\slow\}}\, \boldsymbol{\gamma}^{\{\slow,\slow\}}\,\mathbf{1} = 0 \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\fast,1\}}\, \boldsymbol{\gamma}^{\{\fast,\fast,1\}}\,\mathbf{1} = 0 \\
 &&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M  \left[
\boldsymbol{\alpha}^{\{\fast,\fast\}} \, 
\boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}}
+ (M-\lambda) \boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}}
\right]
\,\mathbf{1}
 = 0, 
\\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}}
\, 
\boldsymbol{\gamma}^{\{\slow,\slow\}}\,\mathbf{1}
 = 0, 
\end{eqnarray}
\end{subequations}



\begin{subequations}
\begin{eqnarray}
&&  \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\slow\}}\, \boldsymbol{\gamma}^{\{\slow,\slow\}}\,\mathbf{1} = 0 \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\fast,1\}}\, \boldsymbol{\gamma}^{\{\fast,\fast,1\}}\,\mathbf{1} = 0 \\
 &&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}}
\, 
\boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}}\,\mathbf{1}
 = 0, 
\\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\gamma}^{\{\fast,\slow,\lambda\}}
\, 
\boldsymbol{\gamma}^{\{\slow,\slow\}}\,\mathbf{1}
 = 0, 
\end{eqnarray}
\end{subequations}


If one sets $\boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}}=:\boldsymbol{\gamma}^{\{\fast,\fast,\}}$ for $\lambda=1,\ldots,M$ to reduce linear algebra costs, the order conditions read (with short-hand $\boldsymbol{\gamma}^{\{\fast,\fast,\}}:= \boldsymbol{\gamma}^{\{\fast,\fast,\lambda\}}$), if we assume 
 that both basic ROW-schemes $(\mathbf{b}^{\{\slow\}},\boldsymbol{\alpha}^{\{\slow,\slow\}},\boldsymbol{\gamma}^{\{\slow,\slow\}})$ and $(\mathbf{b}^{\{\fast\}},\boldsymbol{\alpha}^{\{\fast,\fast\}},\boldsymbol{\gamma}^{\{\fast,\fast\}})$ are of order three:

  
\begin{subequations}
  \begin{eqnarray}
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\fast,1\}}\, \boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1} = \frac{M^2}{6} \\
&& \mathbf{b}^{\{\fast\}\,T} \, 
\left( \sum_{\lambda=1}^M \boldsymbol{\alpha}^{\{\fast,\slow,\lambda \}}
\right) \, \boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1} = \frac{M}{6}
\end{eqnarray}
\end{subequations}
%


\begin{subequations}
\begin{eqnarray}
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\fast,1\}}\, \boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1} = 0 \\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\gamma}^{\{\fast,\slow,\lambda\}}
\, 
\boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1}
 = 0, 
\end{eqnarray}
\end{subequations}



\begin{subequations}
\begin{eqnarray}
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\alpha}^{\{\slow,\fast,1\}}\, \boldsymbol{\gamma}^{\{\fast,\fast\}}\,\mathbf{1} = 0 \\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\alpha}^{\{\fast,\slow,\lambda\}}
\, 
\boldsymbol{\gamma}^{\{\slow,\slow\}}\,\mathbf{1}
 = 0, 
\end{eqnarray}
\end{subequations}



\begin{subequations}
\begin{eqnarray}
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\gamma}^{\{\slow,\fast,1\}}\, \boldsymbol{\gamma}^{\{\fast,\fast\}}\,\mathbf{1} = 0 \\
&&
\mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M 
\boldsymbol{\gamma}^{\{\fast,\slow,\lambda\}}
\, 
\boldsymbol{\gamma}^{\{\slow,\slow\}}\,\mathbf{1}
 = 0, 
\end{eqnarray}
\end{subequations}
 
 


==> numerical_experiments.tex <==



\if 0
\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=0.00390625,
xmax=0.1,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-11,
ymax=1e-06,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
title style={font=\bfseries},
title={IMEX-Case Order 3 (stiff Mass-Spring-System, nonlinear F), M=10, $\gamma = 1$},
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.0625	5.68357737077472e-08\\
0.03125	7.12804083584858e-09\\
0.015625	8.936754734534e-10\\
0.0078125	1.1173108631521e-10\\
0.00390625	1.39637730803557e-11\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.0625	3.21386990606075e-07\\
0.03125	4.03178554379967e-08\\
0.015625	5.04875827635906e-09\\
0.0078125	6.31646779074628e-10\\
0.00390625	7.89888317091872e-11\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.03125	3.0517578125e-07\\
0.015625	3.814697265625e-08\\
0.0078125	4.76837158203125e-09\\
};
\addlegendentry{$\mathcal{O}(H^3)$}

\end{axis}
\end{tikzpicture}%

\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=0.00390625,
xmax=0.1,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-11,
ymax=1e-06,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
title style={font=\bfseries},
title={IMIM-Case Order 3 (stiff Mass-Spring-System, nonlinear F), M=10, $\gamma = 1$},
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.0625	5.67901581788757e-08\\
0.03125	7.12626126323526e-09\\
0.015625	8.93699044223017e-10\\
0.0078125	1.11749794324176e-10\\
0.00390625	1.39691418070924e-11\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.0625	2.47659001986686e-07\\
0.03125	3.07805778035432e-08\\
0.015625	3.83942473438192e-09\\
0.0078125	4.79467505401562e-10\\
0.00390625	5.99143895684826e-11\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.03125	3.0517578125e-07\\
0.015625	3.814697265625e-08\\
0.0078125	4.76837158203125e-09\\
};
\addlegendentry{$\mathcal{O}(H^3)$}

\end{axis}
\end{tikzpicture}%

\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=0.00390625,
xmax=0.1,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-11,
ymax=1e-06,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
title style={font=\bfseries},
title={IMEX-Case Order 3 (stiff Mass-Spring-System, nonlinear F), M=10, $\gamma = 1$ (time-lagged Jacobian)},
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.0625	1.52544599803715e-07\\
0.03125	2.04427874222007e-08\\
0.015625	2.65137195122903e-09\\
0.0078125	3.37648883155707e-10\\
0.00390625	4.26077311952017e-11\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.0625	3.70235120982525e-07\\
0.03125	4.54396775857575e-08\\
0.015625	5.62771558820338e-09\\
0.0078125	7.00051907140769e-10\\
0.00390625	8.72820331186091e-11\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.03125	3.0517578125e-07\\
0.015625	3.814697265625e-08\\
0.0078125	4.76837158203125e-09\\
};
\addlegendentry{$\mathcal{O}(H^3)$}

\end{axis}

\begin{axis}[%
width=7.778in,
height=5.833in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%

\begin{tikzpicture}

\begin{axis}[%
width=6.028in,
height=4.754in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=0.00390625,
xmax=0.1,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-11,
ymax=1e-06,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
title style={font=\bfseries},
title={IMIM-Case Order 3 (stiff Mass-Spring-System, nonlinear F), M=10, $\gamma = 1$ (time-lagged Jacobian)},
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.0625	1.52110558258396e-07\\
0.03125	2.04097664181381e-08\\
0.015625	2.64875390153664e-09\\
0.0078125	3.37423879380785e-10\\
0.00390625	4.25855889594344e-11\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.0625	8.96768558208696e-07\\
0.03125	1.05666475178349e-07\\
0.015625	1.28081716059733e-08\\
0.0078125	1.57780413162929e-09\\
0.00390625	1.95890633788e-10\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.03125	3.0517578125e-07\\
0.015625	3.814697265625e-08\\
0.0078125	4.76837158203125e-09\\
};
\addlegendentry{$\mathcal{O}(H^3)$}

\end{axis}

\begin{axis}[%
width=7.778in,
height=5.833in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
\fi 

\begin{comment}
\subsection{Order conditions for Multirate GARK-ROW schemes}
The order conditions of Multirate GARK-ROW schemes can be obtained by applying the GARK-ROW order conditions~\eqref{eqn:GARK-ROW-order3-conditions} on them  as an instant of a partitioned GARK-ROW scheme. Order conditions up to order three are given in the appendix.
\if 0
We apply now the GARK-ROW order conditions~\eqref{eqn:GARK-ROW-order3-conditions} on Multirate GARK-ROW schemes as an instant of a partitioned GARK-ROW scheme. The order one conditions read for order one
\begin{subequations}
\label{eqn:multirate-GARK-ROW-order3-conditions}
\begin{eqnarray}
&& \b\S*  \, \one = 1,  \\
                         && \b\F*  \, \one = 1, 
                         \end{eqnarray}
\end{subequations}                         
for order 2 we get
\begin{subequations}
\begin{eqnarray}
&&
\b\S*  \, \boldsymbol{\alpha}\SS \, \one = \frac{1}{2}, \\
&&\b\S*  \, \boldsymbol{\alpha}\SFL[1] \, \one = \sfrac{\mratio}{2},\\
&&\b\F*  \, 
 \boldsymbol{\alpha}\FF 
 \, \one = \frac{1}{2}, \\
&&\b\F*  \, \left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\alpha}\FSL[\lambda] \right) \, \one = \sfrac{\mratio}{2},\\
&&
\b\S*  \, \boldsymbol{\gamma}\SS \, \one = 0, \\
&&\b\S*  \, \boldsymbol{\gamma}\SFL[1] \, \one = 0,\\
&&\b\F*  \, \left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\gamma}\FFL[\lambda]\right) \, \one = 0,\\
&&\b\F*  \, \left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\gamma}\FSL[\lambda] \right) \, \one = 0,
\end{eqnarray}
and for order 3
\begin{eqnarray}
 &&
%\begin{cases}
\b\S*  \, \bigl( (\boldsymbol{\alpha}\SS\,\one )\times (\boldsymbol{\alpha}\SS\,\one ) \bigr) = \frac{1}{3}, \\
&& \b\S*  \, \bigl( (\boldsymbol{\alpha}\SS\,\one )\times (\boldsymbol{\alpha}\SFL[1]\,\one ) \bigr) = \sfrac{\mratio}{3}, \\
&& \b\S*  \, \bigl( (\boldsymbol{\alpha}\SFL[1]\,\one )\times (\boldsymbol{\alpha}\SS\,\one ) \bigr) = \sfrac{\mratio}{3}, \\
&& \b\S*  \, \bigl( (\boldsymbol{\alpha}\SFL[1]\,\one )\times (\boldsymbol{\alpha}\SFL[1]\,\one ) \bigr) = \sfrac{\mratio^2}{3}, \\
&&
%\b\F*  \, \bigl( (\boldsymbol{\alpha}\FF\,\one )\times (\boldsymbol{\alpha}\FF\,\one ) 
%- \sfrac{\mratio-1}{\mratio} \sum_{\lambda=1}^{\mratio}  \boldsymbol{\gamma}^{\{\fast,\fast,\lambda \}}\,\one 
%\bigr) = \frac{1}{3}, \\
\b\F*  \, \bigl( (\boldsymbol{\alpha}\FF\,\one )\times (\boldsymbol{\alpha}\FF\,\one ) 
= \frac{1}{3}, \\
&& \b\F*  \,  \sum_{\lambda=1}^{\mratio}  
\Bigl( 
\left( \boldsymbol{\alpha}\FF\,\one 
\right) \times 
\left( \boldsymbol{\alpha}\FSL[\lambda] \,\one 
 \right)
+ (\lambda-1) \boldsymbol{\alpha}\FSL[\lambda]
\,\one 
\Bigr)  
  =  \sfrac{\mratio^2}{3}, \\
%&& \b\F*  \, \Bigl( \sum_{\lambda=1}^{\mratio}  \left( \boldsymbol{\alpha}\FF\,
% \boldsymbol{\alpha}\FSL[\lambda] 
%+ (\lambda-1) \boldsymbol{\alpha}\FSL[\lambda] \right)
%\Bigr)  \,\one   =  \sfrac{\mratio^2}{3}, \\
%&& \b\F*  \, \Bigl( \sum_{\lambda=1}^{\mratio}  \left( \boldsymbol{\alpha}\FSL[\lambda]\,
% \boldsymbol{\alpha}\FF 
%+ (\lambda-1) \boldsymbol{\alpha}\FSL[\lambda] \right)
%\Bigr)  \,\one   =  \sfrac{\mratio^2}{3}, \\
&& \b\F*  \,  \sum_{\lambda=1}^{\mratio}  
\Bigl( 
\left( \boldsymbol{\alpha}\FSL[\lambda]\,\one 
\right) \times 
\left( \boldsymbol{\alpha}\FF \,\one 
 \right)
+ (\lambda-1) \boldsymbol{\alpha}\FSL[\lambda]
\,\one 
\Bigr)  
  =  \sfrac{\mratio^2}{3}
 \\
&& \b\F*  \, \sum_{\lambda=1}^{\mratio} \bigl( (\boldsymbol{\alpha}\FSL[\lambda]\,\one )\times (\boldsymbol{\alpha}\FSL[\lambda]\,\one ) \bigr) = \sfrac{\mratio}{3}, 
  \end{eqnarray}
  \end{subequations}
  
\begin{subequations}
  \begin{eqnarray}
&&  \b\S*  \, \boldsymbol{\alpha}\SS\, \boldsymbol{\alpha}\SS\,\one  = \frac{1}{6} \\
&& \b\S*  \, \boldsymbol{\alpha}\SS\, \boldsymbol{\alpha}\SFL[1]\,\one  = \sfrac{\mratio}{6} \\
&& \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\alpha}\FSL[1]\,\one  = \sfrac{\mratio}{6} \\
&& \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\alpha}\FF\,\one  = \sfrac{\mratio^2}{6} \\
&&  \b\F*  \, \boldsymbol{\alpha}\FF\, \boldsymbol{\alpha}^{\{\fast,\fast,\}}\,\one  = \frac{1}{6} \\
&& \b\F*  \, \left(
\sum_{\lambda=1}^{\mratio} \boldsymbol{\alpha}\FF\, \boldsymbol{\alpha}\FSL[\lambda] +
 \sum_{\lambda=1}^{\mratio-1} (\mratio-\lambda) \boldsymbol{\alpha}\FSL[\lambda]
\right) \,\one  = \sfrac{\mratio^2}{6} \\
&& \b\F*  \, 
\left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\alpha}\FSL[\lambda]
\right) \, 
 \boldsymbol{\alpha}\SFL[1]
 \,\one  = \sfrac{\mratio^2}{6} \\
&& \b\F*  \, 
\left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\alpha}^{\{\fast,\slow,\lambda \}}
\right) \, \boldsymbol{\alpha}\SS\,\one  = \sfrac{\mratio}{6}
\end{eqnarray}
\end{subequations}
%


\begin{subequations}
\begin{eqnarray}
&&
%\begin{cases}
 \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\alpha}\SS\,\one  = 0 \\
&& \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\alpha}\SFL[1]\,\one  = 0 \\
&& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\alpha}\FSL[1]\,\one  = 0 \\
&& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\alpha}\FF\,\one  = 0 \\
&&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FFL[\lambda]
\, 
\boldsymbol{\alpha}\FF %+ (\lambda-1) ]
\,\one 
 = 0, 
\\
&&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FFL[\lambda]
\, 
\boldsymbol{\alpha}\FSL[\lambda]\,\one 
 = 0, 
\\
&&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FSL[\lambda]
\, 
\boldsymbol{\alpha}\SFL[1]\,\one 
 = 0, 
\\
&&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FSL[\lambda]
\, 
\boldsymbol{\alpha}\SS\,\one 
 = 0, 
\end{eqnarray}
\end{subequations}



\begin{subequations}
\begin{eqnarray}
&&  \b\S*  \, \boldsymbol{\alpha}\SS\, \boldsymbol{\gamma}\SS\,\one  = 0 \\
&& \b\S*  \, \boldsymbol{\alpha}\SS\, \boldsymbol{\gamma}\SFL[1]\,\one  = 0 \\
&& \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\gamma}\FSL[1]\,\one  = 0 \\
&& \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\gamma}\FFL[1]\,\one  = 0 \\
 &&
\b\F*  \, \sum_{\lambda=1}^{\mratio}  \left[
\boldsymbol{\alpha}\FF \, 
\boldsymbol{\gamma}\FFL[\lambda]
+ (\mratio-\lambda) \boldsymbol{\gamma}\FFL[\lambda]
\right]
\,\one 
 = 0, 
\\
&&
\b\F*  \, \sum_{\lambda=1}^{\mratio}  \left[
\boldsymbol{\alpha}\FF \, 
\boldsymbol{\gamma}\FSL[1]
+ (\mratio-\lambda) \boldsymbol{\gamma}\FSL[1]
\right]
\,\one 
 = 0, 
\\
&&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\alpha}\FSL[\lambda]
\, 
\boldsymbol{\gamma}\SFL[1]\,\one 
 = 0, 
\\
&&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\alpha}\FSL[\lambda]
\, 
\boldsymbol{\gamma}\SS\,\one 
 = 0, 
\end{eqnarray}
\end{subequations}



\begin{subequations}
\begin{eqnarray}
&&  \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\gamma}\SS\,\one  = 0 \\
&& \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\gamma}\SFL[1]\,\one  = 0 \\
&& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\gamma}\FSL[1]\,\one  = 0 \\
&& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\gamma}\FFL[1]\,\one  = 0 \\
 &&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FFL[\lambda]
\, 
\boldsymbol{\gamma}\FFL[\lambda]\,\one 
 = 0, 
\\
&&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FFL[\lambda]
\, 
\boldsymbol{\gamma}\FSL[\lambda]\,\one 
 = 0, 
\\
&&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FSL[\lambda]
\, 
\boldsymbol{\gamma}\SFL[1]\,\one 
 = 0, 
\\
&&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FSL[\lambda]
\, 
\boldsymbol{\gamma}\SS\,\one 
 = 0, 
\end{eqnarray}
\end{subequations}
\fi
Again, the number of order conditions can be significantly  by assuming internal consistency 
%
\begin{eqnarray*} 
\boldsymbol{\alpha}\FF \,\one  + (\lambda-1) \,\one  & = & \mratio \cdot   \boldsymbol{\alpha}\FSL[\lambda]\,\one , \\
\boldsymbol{\gamma}\FFL[\lambda]\,\one   & = & \mratio \cdot   \boldsymbol{\gamma}\FSL[\lambda]\,\one , \\
\boldsymbol{\alpha}\SFL[1] \,\one  & = & \mratio \cdot  \boldsymbol{\alpha}\SS \,\one , \\
\boldsymbol{\gamma}\SFL[1] \,\one  & = & \mratio \cdot  \boldsymbol{\gamma}\SS \,\one ,
\end{eqnarray*}
%
and the same order-three base scheme $(\b,\boldsymbol{\alpha})$ for both parts:
$(\b\S ,\boldsymbol{\alpha}\SS,\boldsymbol{\gamma}\SS)$ 
for the slow part,   $(\b\F ,\boldsymbol{\alpha}\FF,\boldsymbol{\gamma}\FFL[1])$ for the first step of the fast part and $(\b\F ,\boldsymbol{\alpha}\FF,\boldsymbol{\gamma}\FFL[\lambda])$ ($\lambda=2,\ldots,\mratio$) for the remaining steps.

Now all order two conditions are automatically fullfilled, and only the following order three conditions have to be fulfilled to get order three:
%
%
%
%$$
%(\b,\boldsymbol{\alpha})=(\b\S ,\boldsymbol{\alpha}\SS), \qquad
%(\b,\boldsymbol{\alpha})=(\b\F ,\boldsymbol{\alpha}\FF).
%$$
%Now only the two order-2 conditions
%\begin{subequations}
%\begin{eqnarray}
%&&
%\b\S*  \, \boldsymbol{\gamma}\SS \, \one = 0, \\
%&&\b\F*  \, \left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\gamma}\FFL[\lambda]%\right) \, \one = 0,
%\end{eqnarray}
%\end{subequations}
%remain, and for order three  
\begin{subequations}
 \label{order-mgark-row12}
\begin{eqnarray}
 &&
 \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\alpha}\FF\,\one  = \sfrac{\mratio^2}{6} 
 \label{order-mgark-row11}
   \\
&& \b\F*  \, 
\left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\alpha}\FSL[\lambda]
\right) \, 
 \boldsymbol{\alpha}\SS
 \,\one  = \sfrac{\mratio}{6} \\
%
%\end{eqnarray}
%\end{subequations}
%
%\begin{subequations}
%\begin{eqnarray}
%&&
%\begin{cases}
% \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\alpha}\SS\,\one  = 0 \\
%&& \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\alpha}\SFL[1]\,\one  = 0 \\
%&& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\alpha}\FSL[1]\,\one  = 0 \\
&& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\alpha}\FF\,\one  = 0 \\
%&&
%\b\F*  \, \sum_{\lambda=1}^{\mratio} 
%(\lambda-1) \boldsymbol{\gamma}\FFL[\lambda]
%(\lambda-1) \boldsymbol{\gamma}\FFL[\lambda]
%\, 
%\boldsymbol{\alpha}\FF %+ (\lambda-1) ]
%\,\one 
% = 0, 
%\\
%&&
%\b\F*  \, \sum_{\lambda=1}^{\mratio} 
%\boldsymbol{\gamma}\FFL[\lambda]
%\, 
%\boldsymbol{\alpha}\FF\,\one 
 %= 0, 
%\\
%&&
%\b\F*  \, \sum_{\lambda=1}^{\mratio} 
%\boldsymbol{\gamma}\FSL[\lambda]
%\, 
%\boldsymbol{\alpha}\SFL[1]\,\one 
% = 0, 
%\\
&&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FSL[\lambda]
\, 
\boldsymbol{\alpha}\SS\,\one 
 = 0 \\
%\end{eqnarray}
%\end{subequations}
%
%
%
%\begin{subequations}
%\begin{eqnarray}
%&&  \b\S*  \, \boldsymbol{\alpha}\SS\, \boldsymbol{\gamma}\SS\,\one  = 0 \\
%&& \b\S*  \, \boldsymbol{\alpha}\SS\, \boldsymbol{\gamma}\SFL[1]\,\one  = 0 \\
%&& \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\gamma}\FSL[1]\,\one  = 0 \\
&& \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\gamma}\FFL[1]\,\one  = 0 \\
 %&&
%\b\F*  \, \sum_{\lambda=1}^{\mratio}  %\left[
%\boldsymbol{\alpha}\FF \, 
%\boldsymbol{\gamma}\FFL[\lambda]
%+ (\mratio-\lambda) \boldsymbol{\gamma}\FFL[\lambda]
%\right]
%\,\one 
% = 0, 
%\\
%&&
%\b\F*  \,  %\left[
%\boldsymbol{\alpha}\FF \, 
%\boldsymbol{\gamma}\FFL[1]
%+ (\mratio-\lambda) \boldsymbol{\gamma}\FFL[\lambda]
%\right]
%\,\one 
% = 0, 
%\\
%&&
%\b\F*  \, \sum_{\lambda=1}^{\mratio}  \left[
%\boldsymbol{\alpha}\FF \, 
%\boldsymbol{\gamma}\FSL[1]
%+ (\mratio-\lambda) \boldsymbol{\gamma}\FSL[1]
%\right]
%\,\one 
% = 0, 
%\\
%&&
%\b\F*  \, \sum_{\lambda=1}^{\mratio} 
%\boldsymbol{\alpha}\FSL[\lambda]
%\, 
%\boldsymbol{\gamma}\SFL[1]\,\one 
% = 0, 
%\\
&&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\alpha}\FSL[\lambda]
\, 
\boldsymbol{\gamma}\SS\,\one 
 = 0 \\ 
%\end{eqnarray}
%\end{subequations}
%
%
%
%\begin{subequations}
%\begin{eqnarray}
%&&  \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\gamma}\SS\,\one  = 0 \\
%&& \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\gamma}\SFL[1]\,\one  = 0 \\
%&& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\gamma}\FSL[1]\,\one  = 0 \\
&& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\gamma}\FFL[1]\,\one  = 0 \\
% &&
%\b\F*  \, \sum_{\lambda=1}^{\mratio} 
%\boldsymbol{\gamma}\FFL[\lambda]
%\, 
%boldsymbol{\gamma}\FFL[\lambda]\,\one 
% = 0, 
%\\
%&&
%\b\F*  \, \sum_{\lambda=1}^{\mratio} 
%\boldsymbol{\gamma}\FFL[\lambda]
%\, 
%\boldsymbol{\gamma}\FSL[\lambda]\,\one 
% = 0, 
%\\
%&&
%\b\F*  \, \sum_{\lambda=1}^{\mratio} 
%\boldsymbol{\gamma}\FSL[\lambda]
%\, 
%\boldsymbol{\gamma}\SFL[1]\,\one 
% = 0, 
%\\
&&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FSL[\lambda]
\, 
\boldsymbol{\gamma}\SS\,\one 
 = 0, 
\end{eqnarray}
\end{subequations}
\end{comment}

\ifnum \value{book}=0
\begin{comment}
\fi

\section{Numerical results}

As a first  example of a system with component-wise multiscale behavior we consider a mathematical pendulum of constant length $\ell$ that is coupled to a damped  oscillator with a horizontal degree of freedom, as illustrated in Figure~\ref{fig:coupled-pendulum}. 
%, taken from~\cite{Arnold_2007_MR-multibody}. \textcolor{red}{The figure and the reference are not here.} 
The system consists of two rigid bodies: the first mass $m_{\rm{pend}}$ is connected to a second mass $m_{\rm{osc}}$ by a soft spring. 

\begin{figure}
%\centerline{\includegraphics[width=0.7\textwidth]{Figures/pendulum_adnotated.pdf}}
\centering
\setlength{\unitlength}{1cm}
\scalebox{0.75}{
\begin{picture}(20,5)
\put(4.5,3.2){\Large{$\alpha$}}
\put(4.5,4.8){\Large{$x_2$}}
\put(9.2,3.6){\Large{$x_1$}}
\put(3.,2.8){\Large{$g$}}
\put(6.5,0.8){\Large{$m_{\rm{pend}}$}}
\put(9.2,0.8){\Large{$m_{\rm{osc}}$}}
\put(6.,2.7){\Large{$\ell$}}
\put(7.99,2.0){\Large{$k,\,d$}}
\put(2.5,0){\includegraphics[width=2.9in]{Figures/pendulum.eps}}
\end{picture}
}
\caption{Mathematical pendulum coupled to an oscillator (taken after~\cite{Arnold_2007_MR-multibody}).
}
\label{fig:coupled-pendulum} 
\end{figure}

The minimal set of coordinates $\y=[\alpha,x_1]^T$  uniquely describe the position of both bodies. The equations of motion given by the Euler-Lagrange equation~\cite{Arnold_2007_MR-multibody} read:
%
\begin{eqnarray*}
\ddot{\y} & = & \funs(\y) + \funf(\y)
\end{eqnarray*}
with
\begin{align*}
\funs(\y)= \begin{pmatrix} 
\frac{\cos (\y_1)F}{m_{\rm{pend}}l} \\ - \frac{F}{m_{\rm{osc}}}
\end{pmatrix}
\quad & \mbox{and} \quad \funf(q) = \begin{pmatrix} 
- g \sin (\y_1) \\ 0 \end{pmatrix}
    \end{align*}
and the nonlinear spring-damper force $F$ modeled by
%
\[
F= k \, \big(\y_2 - \ell\, \sin(\y_1) \big) \big|y_2 - \ell\, \sin(\y_1) \big| + d \, 
\big(\dot y_2 - \ell\, \dot y_2\, \cos (\y_1) \big) \big|\dot y_2 - \ell\, \dot y_2\, \cos (\y_1) \big|,
\]
%
where $k$ denotes the spring stiffness and $d$ is the coefficient of friction. 

Here $\funf$ defines a fast changing process that is inexpensive to evaluate, whereas $\funs$ is a slowly changing process, but is expensive to evaluate. The multirate potential lies in evaluating the cheap and fast part  $\funf$ more often then the slow and expensive part $\funs$.
As seen in Figure~\ref{fig:forces.twobody}, $\funf$ defines a fast changing force, whereas $\funs$ is slowly changing. 
%
\begin{figure}
  \centering
  \subfloat[Components of slow force $\funs(t,\y(t))$\label{fig:forces.twobody.a}]{
  \includegraphics[width=0.45\textwidth,height=0.3\textwidth]{Figures/Twobody_force1.eps}}
  \subfloat[Fast force (1st component of $\funf(t,\y(t))$)\label{fig:forces.twobody.b}]{
  \includegraphics[width=0.45\textwidth,height=0.3\textwidth]{Figures/Twobody_force2.eps}}            
\caption{Time evolution of slow and fast forces acting on the two-body system.}
\label{fig:forces.twobody} 
\end{figure}

This two-dimensional second order system of differential equations can be easily transformed into a four-dimensional ODE system by introducing the derivatives of $\y$ as additional unknowns. 

The numerical results for both the IMIM and IMEX embedded scheme of order (2)3 of Chapter 5.2 for exact Jacobian (MGARK ROS schemes) and inexact Jacobian can be found in figures~\ref{imim.order3} and~\ref{imim.order2} and figures~\ref{imex.order3} and~\ref{imex.order2}, resp. In all cases, order three (and order two for the embedded scheme) of the methods is nicely verified. 

\begin{figure}[htb]
\centering
  \begin{minipage}[t]{.45\linewidth}
\begin{tikzpicture}
%
\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(0.903in,0.465in)},
scale only axis,
xmode=log,
xmin=0.0078125,
xmax=0.125,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-09,
ymax=0.0001,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(0,1)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.125	6.94162308998861e-06\\
0.0625	1.03364956705403e-06\\
0.03125	1.45750384147302e-07\\
0.015625	1.72627387933067e-08\\
0.0078125	2.31320931607263e-09\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.125	2.81930088363815e-05\\
0.0625	3.49101323714807e-06\\
0.03125	4.34184650410408e-07\\
0.015625	5.39556564378624e-08\\
0.0078125	6.75576148473714e-09\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.0625	2.44140625e-07\\
0.03125	3.0517578125e-08\\
0.015625	3.814697265625e-09\\
};
\addlegendentry{$\mathcal{O}(H^3)$}

\end{axis}
\end{tikzpicture}%
  %\subcaption{exact Jacobian}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{.45\linewidth}
\begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(0.903in,0.465in)},
scale only axis,
xmode=log,
xmin=0.0078125,
xmax=0.125,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-09,
ymax=0.0001,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(0,1)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.125	1.42999030430121e-05\\
0.0625	3.70684906900488e-06\\
0.03125	5.81803061555676e-07\\
0.015625	8.43883232248747e-08\\
0.0078125	1.10319255135835e-08\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.125	3.1008294852583e-05\\
0.0625	3.86901053307893e-06\\
0.03125	4.75597727848613e-07\\
0.015625	5.88169400695742e-08\\
0.0078125	7.16535850017403e-09\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.0625	2.44140625e-07\\
0.03125	3.0517578125e-08\\
0.015625	3.814697265625e-09\\
};
\addlegendentry{$\mathcal{O}(H^3)$}

\end{axis}
\end{tikzpicture}%
  %\subcaption{time-lagged Jacobian}
  \end{minipage}
  
  \caption{\label{imim.order3} IMIM-Case Order 3 with multirate factor $\mratio=10$ and free parameter $\gamma = 1$}
\end{figure}


%%%%% IMIM 2 FIGURE %%%%%
\begin{figure}[htb]
\centering
  \begin{minipage}[t]{.45\linewidth}
  \begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(0.903in,0.465in)},
scale only axis,
xmode=log,
xmin=0.001953125,
xmax=0.03125,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-09,
ymax=1e-05,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(0,1)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.03125	1.72715197761354e-06\\
0.015625	4.57008072367246e-07\\
0.0078125	1.16406082725641e-07\\
0.00390625	2.94579194872614e-08\\
0.001953125	7.41045187736918e-09\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.03125	2.23406291184252e-06\\
0.015625	5.49179480573164e-07\\
0.0078125	1.37812263935452e-07\\
0.00390625	3.57304440530125e-08\\
0.001953125	1.02746569632171e-08\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.015625	2.44140625e-07\\
0.0078125	6.103515625e-08\\
0.00390625	1.52587890625e-08\\
};
\addlegendentry{$\mathcal{O}(H^2)$}

\end{axis}
\end{tikzpicture}%
  %\subcaption{exact Jacobian}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{.45\linewidth}
  \begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(0.903in,0.465in)},
scale only axis,
xmode=log,
xmin=0.001953125,
xmax=0.03125,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-09,
ymax=1e-05,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(0,1)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.03125	1.51254269540593e-06\\
0.015625	4.28683236093462e-07\\
0.0078125	1.12864240001983e-07\\
0.00390625	2.90148176979555e-08\\
0.001953125	7.35506317144354e-09\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.03125	2.23794210094368e-06\\
0.015625	5.4915124605749e-07\\
0.0078125	1.37785603651768e-07\\
0.00390625	3.57256245035505e-08\\
0.001953125	1.02739660503943e-08\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.015625	2.44140625e-07\\
0.0078125	6.103515625e-08\\
0.00390625	1.52587890625e-08\\
};
\addlegendentry{$\mathcal{O}(H^2)$}

\end{axis}
\end{tikzpicture}%
  %\subcaption{time-lagged Jacobian}
  \end{minipage}
  
  \caption{\label{imim.order2} IMIM-Case Order 2 with multirate factor $\mratio=10$ and free parameter $\gamma = 1$}
\end{figure}

%%%%% IMEX 3 FIGURE %%%%%
\begin{figure}[htb]
\centering
  \begin{minipage}[t]{.45\linewidth}
  \begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(0.903in,0.465in)},
scale only axis,
xmode=log,
xmin=0.0078125,
xmax=0.125,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-09,
ymax=0.0001,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(0,1)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.125	6.84254371269295e-06\\
0.0625	1.02225925399536e-06\\
0.03125	1.44360824968522e-07\\
0.015625	1.70937203605633e-08\\
0.0078125	2.29205541406465e-09\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.125	1.4429066172873e-05\\
0.0625	1.80899827956243e-06\\
0.03125	2.26154241820953e-07\\
0.015625	2.80651936773617e-08\\
0.0078125	3.68036346376498e-09\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.0625	2.44140625e-07\\
0.03125	3.0517578125e-08\\
0.015625	3.814697265625e-09\\
};
\addlegendentry{$\mathcal{O}(H^3)$}

\end{axis}
\end{tikzpicture}%
  %\subcaption{exact Jacobian}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{.45\linewidth}
  \begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(0.903in,0.465in)},
scale only axis,
xmode=log,
xmin=0.0078125,
xmax=0.125,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-09,
ymax=0.0001,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(0,1)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.125	1.43443976605612e-05\\
0.0625	3.69800916926982e-06\\
0.03125	5.80582988427477e-07\\
0.015625	8.42377929254175e-08\\
0.0078125	1.10133750349889e-08\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.125	1.78288394090161e-05\\
0.0625	2.10614592185345e-06\\
0.03125	2.4981631222462e-07\\
0.015625	3.02242271081008e-08\\
0.0078125	3.61628630024864e-09\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.0625	2.44140625e-07\\
0.03125	3.0517578125e-08\\
0.015625	3.814697265625e-09\\
};
\addlegendentry{$\mathcal{O}(H^3)$}

\end{axis}
\end{tikzpicture}%
  %\subcaption{time-lagged Jacobian}
  \end{minipage}
  
  \caption{\label{imex.order3} IMEX-Case Order 3 with multirate factor $\mratio=10$ and free parameter $\gamma = 1$}
\end{figure}

%%%%% IMEX 2 FIGURE %%%%%
\begin{figure}[htb]
\centering
  \begin{minipage}[t]{.45\linewidth}
\begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(0.903in,0.465in)},
scale only axis,
xmode=log,
xmin=0.001953125,
xmax=0.03125,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-09,
ymax=0.1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(0,1)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.03125	1.75026852265367e-06\\
0.015625	4.63440895768719e-07\\
0.0078125	1.18039794709532e-07\\
0.00390625	2.98739021271646e-08\\
0.001953125	7.51568743450605e-09\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.03125	0.000226253086521107\\
0.015625	5.65587618041086e-05\\
0.0078125	1.41402131833715e-05\\
0.00390625	3.53630202351805e-06\\
0.001953125	8.854188193399e-07\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.015625	2.44140625e-05\\
0.0078125	6.103515625e-06\\
0.00390625	1.52587890625e-06\\
};
\addlegendentry{$\mathcal{O}(H^2)$}

\end{axis}
\end{tikzpicture}%
  %\subcaption{exact Jacobian}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{.45\linewidth}
\begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(0.903in,0.465in)},
scale only axis,
xmode=log,
xmin=0.001953125,
xmax=0.03125,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-09,
ymax=0.1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(0,1)}, anchor=north west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.03125	1.51710907510088e-06\\
0.015625	4.33154272127795e-07\\
0.0078125	1.14267556368249e-07\\
0.00390625	2.94030902025425e-08\\
0.001953125	7.456917343986e-09\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.03125	0.000226237973172787\\
0.015625	5.65563059715868e-05\\
0.0078125	1.41398716434155e-05\\
0.00390625	3.53625735007986e-06\\
0.001953125	8.85413134887854e-07\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.015625	2.44140625e-05\\
0.0078125	6.103515625e-06\\
0.00390625	1.52587890625e-06\\
};
\addlegendentry{$\mathcal{O}(H^2)$}

\end{axis}
\end{tikzpicture}%
  %\subcaption{time-lagged Jacobian}
  \end{minipage}
  
  \caption{\label{imex.order2} IMEX-Case Order 2 with multirate factor $\mratio=10$ and free parameter $\gamma = 1$}
\end{figure}


\if 0
\begin{figure}[ht]
    \centering
    \begin{adjustbox}{scale=1}
        \begin{circuitikz}[scale = 0.7]
        \draw
        (0.2,0) to[european voltage source, l=v(t), -] (0.2,2)
        (0.2,2) to[short] (0.2,4)
        (2,3.75) node[plain amp, scale = 0.35] (opamp) {}
        (0.2,4) node[label={above:$u_1$}] {}
        to[short,*-] (opamp.-)
        (opamp.+) to[short] (1,3.5) to[short] (1,0)
        (opamp.out) to[short] (3,3.75) node[label={above:$u_2$}] {}
        to[R,l_=$R(T)$, *-*]
        (5,3.75) node[label={above:$u_3$}] {}
        to[D,-*] 
        (7,3.75) node[label={above:$u_4$}] {}
        to[C,l_=$C$,*-] (7,0) 
        (7,3.75) to[short] (9,3.75) to[R,l=$R_L$] (9,0)
        (0,0) to[short] (9.2,0)
        ;
        %
        \end{circuitikz}
        \end{adjustbox}
    \caption{Electric description of the benchmark circuit.}
\label{fig:circuit}
\end{figure}
\fi 
%\noindent
As a second example, we consider a quasilinear Prothero-Robinson like structure, which can be written as a component split system:
\begin{align*}
\dot y & = A (y-f) + \dot f, \quad y(0)=y_0 \quad \mbox{ with }
    \end{align*}
    \begin{align*}
        \y : =  \begin{pmatrix} \ys \\  \yf
    \end{pmatrix}, \quad
    A \coloneqq   \begin{pmatrix}
    \lambda_1 \ys & \epsilon \\ \epsilon & \lambda_2 \yf
    \end{pmatrix}, \quad
    f \coloneqq  \begin{pmatrix}
    \sin(2 \pi t) +2\\ \sin(10 \cdot 2 \pi t) +2
    \end{pmatrix}, \quad
    y_0 \coloneqq  \begin{pmatrix} 2 \\ 2
    \end{pmatrix},
    \end{align*}
    i.e., the exact solution is given by $y=f$. The numerical results for $\lambda_1=-10^{-6}$, $\lambda_1=-1$ $\epsilon=5 \cdot 10^{-4}$ on the time interval $[0,2]$ are given in ...

%%%%% IMIM 3 FIGURE %%%%%
\begin{figure}[hbt]
\centering
  \begin{minipage}[t]{.45\linewidth}
\begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1/(2^13),
xmax=0.001953125,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-13,
ymax=0.001,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(1,0)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.001953125	0.000145660051827701\\
0.0009765625	1.89153614291726e-05\\
0.00048828125	2.41188778282719e-06\\
0.000244140625	3.04559166774965e-07\\
0.0001220703125	3.82653970731894e-08\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.001953125	4.51894092368121e-07\\
0.0009765625	6.41687210034547e-08\\
0.00048828125	8.4782043607845e-09\\
0.000244140625	1.08753894778602e-09\\
0.0001220703125	1.3763701289804e-10\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.0009765625	1.86264514923096e-07\\
0.00048828125	2.3283064365387e-08\\
0.000244140625	2.91038304567337e-09\\
};
\addlegendentry{$\mathcal{O}(H^3)$}

\end{axis}

\begin{axis}[%
width=7.778in,
height=5.833in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
    %\subcaption{exact Jacobian}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{.45\linewidth}
  \begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1/(2^13),
xmax=0.001953125,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-13,
ymax=0.01,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(1,0)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.001953125	0.0025089202791917\\
0.0009765625	0.000335765787175646\\
0.00048828125	4.32789618649565e-05\\
0.000244140625	5.48847382431106e-06\\
0.0001220703125	6.9089909171538e-07\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.001953125	7.75947104791896e-06\\
0.0009765625	1.12364210425042e-06\\
0.00048828125	1.54588006395784e-07\\
0.000244140625	2.02984744568369e-08\\
0.0001220703125	2.64227706381348e-09\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.0009765625	1.86264514923096e-07\\
0.00048828125	2.3283064365387e-08\\
0.000244140625	2.91038304567337e-09\\
};
\addlegendentry{$\mathcal{O}(H^3)$}

\end{axis}

\begin{axis}[%
width=7.778in,
height=5.833in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
  %\subcaption{time-lagged Jacobian}
  \end{minipage}
  \caption{Prothero-Robinson, IMIM-Case Order 3 with multirate factor $M=10$}
\end{figure}

%%%%% IMIM 2 FIGURE %%%%%

\begin{figure}[htb]
\centering
  \begin{minipage}[t]{.45\linewidth}
\begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1/(2^16),
xmax=0.000244140625,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=9.99999999999996e-13,
ymax=9.99999999999998e-05,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(1,0)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.000244140625	1.16644425678381e-05\\
0.0001220703125	2.91937646590412e-06\\
6.103515625e-05	7.30250663050214e-07\\
3.0517578125e-05	1.82613389743125e-07\\
1.52587890625e-05	4.56596778164453e-08\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.000244140625	1.67533327211089e-07\\
0.0001220703125	4.20295305225693e-08\\
6.103515625e-05	1.05252100368602e-08\\
3.0517578125e-05	2.63350186102684e-09\\
1.52587890625e-05	6.58645582518602e-10\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.0001220703125	1.49011611938477e-07\\
6.103515625e-05	3.72529029846191e-08\\
3.0517578125e-05	9.31322574615479e-9\\
};
\addlegendentry{$\mathcal{O}(H^2)$}

\end{axis}

\begin{axis}[%
width=7.778in,
height=5.833in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
    %\subcaption{exact Jacobian}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{.45\linewidth}
  \begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1/(2^16),
xmax=0.000244140625,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-12,
ymax=0.0001,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(1,0)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.000244140625	1.08513284131639e-05\\
0.0001220703125	2.81668330748275e-06\\
6.103515625e-05	7.17348747958368e-07\\
3.0517578125e-05	1.80996560406044e-07\\
1.52587890625e-05	4.54573356734045e-08\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.000244140625	1.60985834884997e-07\\
0.0001220703125	4.14610115129221e-08\\
6.103515625e-05	1.04601518557956e-08\\
3.0517578125e-05	2.62639066050951e-09\\
1.52587890625e-05	6.57786269897542e-10\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.0001220703125	1.49011611938477e-07\\
6.103515625e-05	3.72529029846191e-08\\
3.0517578125e-05	9.31322574615479e-09\\
};
\addlegendentry{$\mathcal{O}(H^2)$}

\end{axis}

\begin{axis}[%
width=7.778in,
height=5.833in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
  %\subcaption{time-lagged Jacobian}
  \end{minipage}
  \caption{Prothero-Robinson, IMIM-Case Order 2 with multirate factor $M=10$}
\end{figure}

%%%%% IMEX 3 FIGURE %%%%%

\begin{figure}[htb]
\centering
  \begin{minipage}[t]{.45\linewidth}
\begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1/(2^13),
xmax=0.001953125,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-13,
ymax=0.000999999999999999,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(1,0)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.001953125	0.000142604657360046\\
0.0009765625	1.84844487836067e-05\\
0.00048828125	2.35461157016559e-06\\
0.000244140625	2.97175219543533e-07\\
0.0001220703125	3.73280353294092e-08\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.001953125	4.87995882370029e-07\\
0.0009765625	6.38863077995211e-08\\
0.00048828125	8.17872347624871e-09\\
0.000244140625	1.03479314006449e-09\\
0.0001220703125	1.30125688002636e-10\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.0009765625	1.86264514923096e-07\\
0.00048828125	2.3283064365387e-08\\
0.000244140625	2.91038304567337e-09\\
};
\addlegendentry{$\mathcal{O}(H^3)$}

\end{axis}

\begin{axis}[%
width=7.778in,
height=5.833in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
    %\subcaption{exact Jacobian}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{.45\linewidth}
  \begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1/(2^13),
xmax=0.001953125,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-13,
ymax=0.01,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(1,0)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.001953125	0.00249660209898517\\
0.0009765625	0.000333893785256389\\
0.00048828125	4.30214533841955e-05\\
0.000244140625	5.4547529715343e-06\\
0.0001220703125	6.86586618670049e-07\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.001953125	9.54247084150595e-06\\
0.0009765625	1.28219101602767e-06\\
0.00048828125	1.66128603762417e-07\\
0.000244140625	2.11350483780848e-08\\
0.0001220703125	2.66906141632717e-09\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.0009765625	1.86264514923096e-07\\
0.00048828125	2.3283064365387e-08\\
0.000244140625	2.91038304567337e-09\\
};
\addlegendentry{$\mathcal{O}(H^3)$}

\end{axis}

\begin{axis}[%
width=7.778in,
height=5.833in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
  %\subcaption{time-lagged Jacobian}
  \end{minipage}
  \caption{Prothero-Robinson, IMEX-Case Order 3 with multirate factor $M=10$}
\end{figure}

%%%%% IMEX 2 FIGURE %%%%%

\begin{figure}[htb]
\centering
  \begin{minipage}[t]{.45\linewidth}
\begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1/(2^16),
xmax=0.000244140625,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=9.99999999999996e-13,
ymax=9.99999999999998e-05,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(1,0)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.000244140625	1.16382839778773e-05\\
0.0001220703125	2.91588671208487e-06\\
6.103515625e-05	7.29771464147433e-07\\
3.0517578125e-05	1.82543490101494e-07\\
1.52587890625e-05	4.56484419153469e-08\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.000244140625	1.68755740936888e-07\\
0.0001220703125	4.21862171862131e-08\\
6.103515625e-05	1.05462603094963e-08\\
3.0517578125e-05	2.6365296612596e-09\\
1.52587890625e-05	6.5912519886524e-10\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.0001220703125	1.49011611938477e-07\\
6.103515625e-05	3.72529029846191e-08\\
3.0517578125e-05	9.31322574615479e-09\\
};
\addlegendentry{$\mathcal{O}(H^2)$}

\end{axis}

\begin{axis}[%
width=7.778in,
height=5.833in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
    %\subcaption{exact Jacobian}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{.45\linewidth}
  \begin{tikzpicture}

\begin{axis}[%
width=1.8837in,
height=1.18615in,
at={(1.011in,0.642in)},
scale only axis,
xmode=log,
xmin=1/(2^16),
xmax=0.000244140625,
xminorticks=true,
xlabel style={font=\color{white!15!black}},
xlabel={Macro Step Size},
ymode=log,
ymin=1e-12,
ymax=0.0001,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Global Error},
axis background/.style={fill=white},
legend style={at={(1,0)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, mark=square, mark options={solid, red}]
  table[row sep=crcr]{%
0.000244140625	1.07467213421586e-05\\
0.0001220703125	2.80309400402246e-06\\
6.103515625e-05	7.15588779787169e-07\\
3.0517578125e-05	1.80765459933951e-07\\
1.52587890625e-05	4.54259589943717e-08\\
};
\addlegendentry{$y_S$}

\addplot [color=blue, mark=square, mark options={solid, blue}]
  table[row sep=crcr]{%
0.000244140625	1.64896761134514e-07\\
0.0001220703125	4.17245256123522e-08\\
6.103515625e-05	1.04889092966687e-08\\
3.0517578125e-05	2.62944777063012e-09\\
1.52587890625e-05	6.58242349516058e-10\\
};
\addlegendentry{$y_F$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
0.0001220703125	1.49011611938477e-07\\
6.103515625e-05	3.72529029846191e-08\\
3.0517578125e-05	9.31322574615479e-09\\
};
\addlegendentry{$\mathcal{O}(H^2)$}

\end{axis}

\begin{axis}[%
width=7.778in,
height=5.833in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
  %\subcaption{time-lagged Jacobian}
  \end{minipage}
  \caption{Prothero-Robinson, IMEX-Case Order 2 with multirate factor $M=10$}
\end{figure}

\if 0
we consider the thermal-electric benchmark shown in figure~\ref{fig:circuit}.
This circuit consists of an operational amplifier, two resistors,
a diode and a capacitor. 
The resistor $R(T)$ produces and transports heat and is temperature dependent. The amplifier is a heat source and the diode has a temperature dependent characteristic curve. 

The thermal component defines the slow (and non-stiff) part, the electrical component the fast (and stiff) part of the system.

The distributed temperature $T$ of the resistor (wire) is described by the 1-D heat equation, which is semi-discretised using a finite volume approach. Due to the electric current, the resistor is heated and so the resistance of this device changes: $R=R(T)$. The characteristic curve of the diode is also temperature dependent. The voltages are modeled by a nodal analysis using Kirchhoff’s laws. Finally we get a partitioned system of ordinary differential equations like in (1). The vector of unknowns $\y=(u_3,u_4,e,T)^\top$ comprises the voltages $u_3$ and $u_4$ at nodes 3 and 4, resp., the dissipated energy $e$ in the thermally dependent resistor and the vector of temperatures $T$ in the semi-discretised resistor. The multirate behaviour of this system is given by the physical properties: the voltages and the dissipated energy change very fast (due to the source of the network), and the temperature in the resistor changes much slower. Hence the partitioning according to the dynamical behaviour is quite natural:
$$
\ys = T, \quad \yf = \begin{bmatrix} 
u_3 \\ u_4 \\ e
\end{bmatrix}.
$$
The numerical results for both schemes are given in ...











\fi

\ifnum \value{book}=0
\end{comment}
\fi

\ifnum \value{book}=0
\begin{comment}
\fi

\section{Appendix}
Applying the GARK-ROS order conditions~\eqref{eqn:GARK-ROS-order3-conditions} on Multirate GARK-ROS schemes as an instant of a partitioned GARK-ROS scheme yields
\begin{subequations}
\label{order.mr-gark-ros}
\begin{eqnarray}
\hspace*{1cm} \textnormal{order 1:   } && \b\S*  \, \one = 1,  \\
                         && \b\F*  \, \one = 1, 
                         \end{eqnarray}
                         \begin{eqnarray}
\hspace*{1cm} \textnormal{order 2:   } &&
\b\S*  \, \boldsymbol{\beta}\SS \, \one = \frac{1}{2}, \\
&&\b\S*  \, \boldsymbol{\beta}\SFL[1] \, \one = \sfrac{\mratio}{2},\\
&&\b\F*  \, \left(
\sum_{\lambda=1}^{\mratio} \boldsymbol{\beta}\FFL[\lambda]
\right) \, \one = \sfrac{\mratio}{2}, \\
&&\b\F*  \, \left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\beta}\FSL[\lambda] \right) \, \one = \sfrac{\mratio}{2},
\end{eqnarray}
                         \begin{eqnarray}
\hspace*{1cm} 
\textnormal{order 3:   } &&
%\begin{cases}
\b\S*  \, \bigl( (\boldsymbol{\alpha}\SS\,\one )\times (\boldsymbol{\alpha}\SS\,\one ) \bigr) = \frac{1}{3}, \\
&& \b\S*  \, \bigl( (\boldsymbol{\alpha}\SS\,\one )\times (\boldsymbol{\alpha}\SFL[1]\,\one ) \bigr) = \sfrac{\mratio}{3}, \\
%&& \b\S*  \, \bigl( (\boldsymbol{\alpha}\SFL[1]\,\one )\times (\boldsymbol{\alpha}\SS\,\one ) \bigr) = \sfrac{\mratio}{3}, \\
%&& \b\S*  \, \bigl( (\boldsymbol{\alpha}\SFL[1]\,\one )\times (\boldsymbol{\alpha}\SS\,\one ) \bigr) = \sfrac{\mratio}{3}, \\
&& \b\S*  \, \bigl( (\boldsymbol{\alpha}\SFL[1]\,\one )\times (\boldsymbol{\alpha}\SFL[1]\,\one ) \bigr) = \sfrac{\mratio^2}{3}, \\
&&  \b\S*  \, \boldsymbol{\beta}\SS\, \boldsymbol{\beta}\SS\,\one  = \frac{1}{6} \\
&& \b\S*  \, \boldsymbol{\beta}\SS\, \boldsymbol{\beta}\SFL[1]\,\one  = \sfrac{\mratio}{6} \\
&& \b\S*  \, \boldsymbol{\beta}\SFL[1]\, \boldsymbol{\beta}\FSL[1]\,\one  = \sfrac{\mratio}{6} \\
&& \b\S*  \, \boldsymbol{\beta}\SFL[1]\, \boldsymbol{\beta}\FFL[1]\,\one  = \sfrac{\mratio^2}{6} \\
&&
%\begin{cases}
%\b\F*  \, \bigl( (\boldsymbol{\alpha}\FF\,\one )\times (\boldsymbol{\alpha}\FF\,\one ) 
%-(\mratio-1) \boldsymbol{\gamma}\FF\,\one 
%\bigr) = \frac{1}{3}, \\
%&&
\b\F*  \, \bigl( (\boldsymbol{\alpha}\FF\,\one )\times (\boldsymbol{\alpha}\FF\,\one  ) 
+ (\mratio-1) 
   \boldsymbol{\alpha}\FF\,\one 
\bigr) = \frac{3\mratio-1}{6}, \\
&& \b\F*  \,  \sum_{\lambda=1}^{\mratio}  
\Bigl( 
\left( \boldsymbol{\alpha}\FF\,\one 
\right) \times 
\left( \boldsymbol{\alpha}\FSL[\lambda] \,\one 
 \right)
+ (\lambda-1) \boldsymbol{\alpha}\FSL[\lambda]
\,\one 
\Bigr)  
  =  \sfrac{\mratio^2}{3}, \\
%&& \b\F*  \, \Bigl( \sum_{\lambda=1}^{\mratio}  \left( \boldsymbol{\alpha}\FF\,
% \boldsymbol{\alpha}\FSL[\lambda] 
%+ (\lambda-1) \boldsymbol{\alpha}\FSL[\lambda] \right)
%\Bigr)  \,\one   =  \sfrac{\mratio^2}{3}, \\
%&& \b\F*  \, \Bigl( \sum_{\lambda=1}^{\mratio}  \left( \boldsymbol{\alpha}\FSL[\lambda]\,
% \boldsymbol{\alpha}\FF 
%+ (\lambda-1) \boldsymbol{\alpha}\FSL[\lambda] \right)
%\Bigr)  \,\one   =  \sfrac{\mratio^2}{3}, \\
%&& \b\F*  \,  \sum_{\lambda=1}^{\mratio}  
%\Bigl( 
%\left( \boldsymbol{\alpha}\FSL[\lambda]\,\one 
%\right) \times 
%\left( \boldsymbol{\alpha}\FF \,\one 
% \right)
%%+ (\lambda-1) \boldsymbol{\alpha}\FSL[\lambda]
%%\,\one 
%%\Bigr)  
%  =  \sfrac{\mratio^2}{3}, \\
&& \b\F*  \, \sum_{\lambda=1}^{\mratio} \bigl( (\boldsymbol{\alpha}\FSL[\lambda]\,\one )\times (\boldsymbol{\alpha}\FSL[\lambda]\,\one ) \bigr) = \sfrac{\mratio}{3}, \\
&&  \b\F*  \, \sum_{\lambda=1}^{\mratio} \boldsymbol{\beta}\FFL[\lambda]\, \boldsymbol{\beta}\FFL[\lambda]\,\one  = \sfrac{\mratio}{6} \\
&& \b\F*  \, \left(
\sum_{\lambda=1}^{\mratio} \boldsymbol{\beta}\FFL[\lambda]\, \boldsymbol{\beta}\FSL[\lambda] +
 \sum_{\lambda=1}^{\mratio-1} (\mratio-\lambda) \boldsymbol{\beta}\FSL[\lambda]
\right) \,\one  = \sfrac{\mratio^2}{6} \\
&& \b\F*  \, 
\left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\beta}\FSL[\lambda]
\right) \, 
 \boldsymbol{\beta}\SFL[1]
 \,\one  = \sfrac{\mratio^2}{6} \\
&& \b\F*  \, 
\left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\beta}^{\{\fast,\slow,\lambda \}}
\right) \, \boldsymbol{\beta}\SS\,\one  = \sfrac{\mratio}{6}
\end{eqnarray}
\end{subequations}

In a similar way, applying the GARK-ROW order conditions~\eqref{eqn:GARK-ROW-order3-conditions} on Multirate GARK-ROW schemes as an instant of a partitioned GARK-ROW scheme yields the order conditions of Multirate GARK ROW schemes. The order one conditions read for order one
\begin{subequations}
\label{eqn:multirate-GARK-ROW-order3-conditions}
\begin{eqnarray}
&& \b\S*  \, \one = 1,  \\
                         && \b\F*  \, \one = 1, 
                         \end{eqnarray}
\end{subequations}                         
for order 2 we get
\begin{subequations}
\begin{eqnarray}
&&
\b\S*  \, \boldsymbol{\alpha}\SS \, \one = \frac{1}{2}, \\
&&\b\S*  \, \boldsymbol{\alpha}\SFL[1] \, \one = \sfrac{\mratio}{2},\\
&&\b\F*  \, 
 \boldsymbol{\alpha}\FF 
 \, \one = \frac{1}{2}, \\
&&\b\F*  \, \left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\alpha}\FSL[\lambda] \right) \, \one = \sfrac{\mratio}{2},\\
&&
\b\S*  \, \boldsymbol{\gamma}\SS \, \one = 0, \\
&&\b\S*  \, \boldsymbol{\gamma}\SFL[1] \, \one = 0,\\
&&\b\F*  \, \left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\gamma}\FFL[\lambda]\right) \, \one = 0,\\
&&\b\F*  \, \left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\gamma}\FSL[\lambda] \right) \, \one = 0,
\end{eqnarray}
\end{subequations}

and for order 3

\begingroup
\allowdisplaybreaks
%\begin{subequations}
\begin{align*}
&\b\S*  \, \bigl( (\boldsymbol{\alpha}\SS\,\one )\times (\boldsymbol{\alpha}\SS\,\one ) \bigr) = \frac{1}{3},  \\
&\b\S*  \, \bigl( (\boldsymbol{\alpha}\SS\,\one )\times (\boldsymbol{\alpha}\SFL[1]\,\one ) \bigr) = \sfrac{\mratio}{3}, \\
&\b\S*  \, \bigl( (\boldsymbol{\alpha}\SFL[1]\,\one )\times (\boldsymbol{\alpha}\SS\,\one ) \bigr) = \sfrac{\mratio}{3}, \\
 &\b\S*  \, \bigl( (\boldsymbol{\alpha}\SFL[1]\,\one )\times (\boldsymbol{\alpha}\SFL[1]\,\one ) \bigr) = \sfrac{\mratio^2}{3}, \\
 &
\b\F*  \, \bigl( (\boldsymbol{\alpha}\FF\,\one )\times (\boldsymbol{\alpha}\FF\,\one ) 
= \frac{1}{3}, \\
& \b\F*  \,  \sum_{\lambda=1}^{\mratio}  
\Bigl( 
\left( \boldsymbol{\alpha}\FF\,\one 
\right) \times 
\left( \boldsymbol{\alpha}\FSL[\lambda] \,\one 
 \right)
+ (\lambda-1) \boldsymbol{\alpha}\FSL[\lambda]
\,\one 
\Bigr)  
  =  \sfrac{\mratio^2}{3}, \\
& \b\F*  \,  \sum_{\lambda=1}^{\mratio}  
\Bigl( 
\left( \boldsymbol{\alpha}\FSL[\lambda]\,\one 
\right) \times 
\left( \boldsymbol{\alpha}\FF \,\one 
 \right)
+ (\lambda-1) \boldsymbol{\alpha}\FSL[\lambda]
\,\one 
\Bigr)  
  =  \sfrac{\mratio^2}{3}
 \\
 & \b\F*  \, \sum_{\lambda=1}^{\mratio} \bigl( (\boldsymbol{\alpha}\FSL[\lambda]\,\one )\times (\boldsymbol{\alpha}\FSL[\lambda]\,\one ) \bigr) = \sfrac{\mratio}{3}, \\
&  \b\S*  \, \boldsymbol{\alpha}\SS\, \boldsymbol{\alpha}\SS\,\one  = \frac{1}{6} \\
& \b\S*  \, \boldsymbol{\alpha}\SS\, \boldsymbol{\alpha}\SFL[1]\,\one  = \sfrac{\mratio}{6} \\
& \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\alpha}\FSL[1]\,\one  = \sfrac{\mratio}{6} \\
& \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\alpha}\FF\,\one  = \sfrac{\mratio^2}{6} \\
&  \b\F*  \, \boldsymbol{\alpha}\FF\, \boldsymbol{\alpha}^{\{\fast,\fast,\}}\,\one  = \frac{1}{6} \\
& \b\F*  \, \left(
\sum_{\lambda=1}^{\mratio} \boldsymbol{\alpha}\FF\, \boldsymbol{\alpha}\FSL[\lambda] +
 \sum_{\lambda=1}^{\mratio-1} (\mratio-\lambda) \boldsymbol{\alpha}\FSL[\lambda]
\right) \,\one  = \sfrac{\mratio^2}{6} \\
& \b\F*  \, 
\left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\alpha}^{\{\slow,\lambda\}}
\right) \, 
 \boldsymbol{\alpha}\SFL[1]
 \,\one  = \sfrac{\mratio^2}{6} \\
 & \b\F*  \, 
\left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\alpha}^{\{\fast,\slow,\lambda \}}
\right) \, \boldsymbol{\alpha}\SS\,\one  = \sfrac{\mratio}{6} \\
& \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\alpha}\SS\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\alpha}\SFL[1]\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\alpha}\FSL[1]\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\alpha}\FF\,\one  = 0  \\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FFL[\lambda]
\, 
\boldsymbol{\alpha}\FF %+ (\lambda-1) ]
\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FFL[\lambda]
\, 
\boldsymbol{\alpha}\FSL[\lambda]\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FSL[\lambda]
\, 
\boldsymbol{\alpha}\SFL[1]\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FSL[\lambda]
\, 
\boldsymbol{\alpha}\SS\,\one 
 = 0, \\
&  \b\S*  \, \boldsymbol{\alpha}\SS\, \boldsymbol{\gamma}\SS\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\alpha}\SS\, \boldsymbol{\gamma}\SFL[1]\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\gamma}\FSL[1]\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\gamma}\FFL[1]\,\one  = 0 \\
 &
\b\F*  \, \sum_{\lambda=1}^{\mratio}  \left[
\boldsymbol{\alpha}\FF \, 
\boldsymbol{\gamma}\FFL[\lambda]
+ (\mratio-\lambda) \boldsymbol{\gamma}\FFL[\lambda]
\right]
\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio}  \left[
\boldsymbol{\alpha}\FF \, 
\boldsymbol{\gamma}\FSL[1]
+ (\mratio-\lambda) \boldsymbol{\gamma}\FSL[1]
\right]
\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\alpha}\FSL[\lambda]
\, 
\boldsymbol{\gamma}\SFL[1]\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} \boldsymbol{\alpha}\FSL[\lambda]
\, 
\boldsymbol{\gamma}\SS\,\one 
 = 0, \\
&  \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\gamma}\SS\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\gamma}\SFL[1]\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\gamma}\FSL[1]\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\gamma}\FFL[1]\,\one  = 0 \\
 &
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FFL[\lambda]
\, 
\boldsymbol{\gamma}\FFL[\lambda]\,\one 
 = 0, 
\\
& \b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FFL[\lambda]
, 
\boldsymbol{\gamma}\FSL[\lambda]\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FSL[\lambda]\, 
\boldsymbol{\gamma}\SFL[1]\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FSL[\lambda]
\, 
\boldsymbol{\gamma}\SS\,\one 
 = 0, 
 \end{align*}
% \end{subequations}
\endgroup

\if 0
\begin{subequations}
{\allowdisplaybreaks
\begin{align}
&\b\S*  \, \bigl( (\boldsymbol{\alpha}\SS\,\one )\times (\boldsymbol{\alpha}\SS\,\one ) \bigr) = \frac{1}{3}, \\
&\b\S*  \, \bigl( (\boldsymbol{\alpha}\SS\,\one )\times (\boldsymbol{\alpha}\SFL[1]\,\one ) \bigr) = \sfrac{\mratio}{3}, \\
&\b\S*  \, \bigl( (\boldsymbol{\alpha}\SFL[1]\,\one )\times (\boldsymbol{\alpha}\SS\,\one ) \bigr) = \sfrac{\mratio}{3}, \\
 &\b\S*  \, \bigl( (\boldsymbol{\alpha}\SFL[1]\,\one )\times (\boldsymbol{\alpha}\SFL[1]\,\one ) \bigr) = \sfrac{\mratio^2}{3}, \\
%
&
\b\F*  \, \bigl( (\boldsymbol{\alpha}\FF\,\one )\times (\boldsymbol{\alpha}\FF\,\one ) 
= \frac{1}{3}, \\
& \b\F*  \,  \sum_{\lambda=1}^{\mratio}  
\Bigl( 
\left( \boldsymbol{\alpha}\FF\,\one 
\right) \times 
\left( \boldsymbol{\alpha}\FSL[\lambda] \,\one 
 \right)
+ (\lambda-1) \boldsymbol{\alpha}\FSL[\lambda]
\,\one 
\Bigr)  
  =  \sfrac{\mratio^2}{3}, \\
& \b\F*  \,  \sum_{\lambda=1}^{\mratio}  
\Bigl( 
\left( \boldsymbol{\alpha}\FSL[\lambda]\,\one 
\right) \times 
\left( \boldsymbol{\alpha}\FF \,\one 
 \right)
+ (\lambda-1) \boldsymbol{\alpha}\FSL[\lambda]
\,\one 
\Bigr)  
  =  \sfrac{\mratio^2}{3}
 \\
 %
& \b\F*  \, \sum_{\lambda=1}^{\mratio} \bigl( (\boldsymbol{\alpha}\FSL[\lambda]\,\one )\times (\boldsymbol{\alpha}\FSL[\lambda]\,\one ) \bigr) = \sfrac{\mratio}{3}, 
&  \b\S*  \, \boldsymbol{\alpha}\SS\, \boldsymbol{\alpha}\SS\,\one  = \frac{1}{6} \\
& \b\S*  \, \boldsymbol{\alpha}\SS\, \boldsymbol{\alpha}\SFL[1]\,\one  = \sfrac{\mratio}{6} \\
& \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\alpha}\FSL[1]\,\one  = \sfrac{\mratio}{6} \\
& \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\alpha}\FF\,\one  = \sfrac{\mratio^2}{6} \\
&  \b\F*  \, \boldsymbol{\alpha}\FF\, \boldsymbol{\alpha}^{\{\fast,\fast,\}}\,\one  = \frac{1}{6} \\
& \b\F*  \, \left(
\sum_{\lambda=1}^{\mratio} \boldsymbol{\alpha}\FF\, \boldsymbol{\alpha}\FSL[\lambda] +
 \sum_{\lambda=1}^{\mratio-1} (\mratio-\lambda) \boldsymbol{\alpha}\FSL[\lambda]
\right) \,\one  = \sfrac{\mratio^2}{6} \\
& \b\F*  \, 
\left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\alpha}^{\{\slow,\lambda\}}
\right) \, 
 \boldsymbol{\alpha}\SFL[1]
 \,\one  = \sfrac{\mratio^2}{6} \\
 %
& \b\F*  \, 
\left( \sum_{\lambda=1}^{\mratio} \boldsymbol{\alpha}^{\{\fast,\slow,\lambda \}}
\right) \, \boldsymbol{\alpha}\SS\,\one  = \sfrac{\mratio}{6} \\
 \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\alpha}\SS\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\alpha}\SFL[1]\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\alpha}\FSL[1]\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\alpha}\FF\,\one  = 0 \\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FFL[\lambda]
\, 
\boldsymbol{\alpha}\FF %+ (\lambda-1) ]
\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FFL[\lambda]
\, 
\boldsymbol{\alpha}\FSL[\lambda]\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FSL[\lambda]
\, 
\boldsymbol{\alpha}\SFL[1]\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FSL[\lambda]
\, 
\boldsymbol{\alpha}\SS\,\one 
 = 0, \\
&  \b\S*  \, \boldsymbol{\alpha}\SS\, \boldsymbol{\gamma}\SS\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\alpha}\SS\, \boldsymbol{\gamma}\SFL[1]\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\gamma}\FSL[1]\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\alpha}\SFL[1]\, \boldsymbol{\gamma}\FFL[1]\,\one  = 0 \\
 &
\b\F*  \, \sum_{\lambda=1}^{\mratio}  \left[
\boldsymbol{\alpha}\FF \, 
\boldsymbol{\gamma}\FFL[\lambda]
+ (\mratio-\lambda) \boldsymbol{\gamma}\FFL[\lambda]
\right]
\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio}  \left[
\boldsymbol{\alpha}\FF \, 
\boldsymbol{\gamma}\FSL[1]
+ (\mratio-\lambda) \boldsymbol{\gamma}\FSL[1]
\right]
\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\alpha}\FSL[\lambda]
\, 
\boldsymbol{\gamma}\SFL[1]\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\alpha}\FSL[\lambda]
\, 
\boldsymbol{\gamma}\SS\,\one 
 = 0, \\
&  \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\gamma}\SS\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\gamma}\SS\, \boldsymbol{\gamma}\SFL[1]\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\gamma}\FSL[1]\,\one  = 0 \\
& \b\S*  \, \boldsymbol{\gamma}\SFL[1]\, \boldsymbol{\gamma}\FFL[1]\,\one  = 0 \\
 &
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FFL[\lambda]
\, 
\boldsymbol{\gamma}\FFL[\lambda]\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FFL[\lambda]
\, 
\boldsymbol{\gamma}\FSL[\lambda]\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FSL[\lambda]
\, 
\boldsymbol{\gamma}\SFL[1]\,\one 
 = 0, 
\\
&
\b\F*  \, \sum_{\lambda=1}^{\mratio} 
\boldsymbol{\gamma}\FSL[\lambda]
\, 
\boldsymbol{\gamma}\SS\,\one 
 = 0, 
\end{align}
}
\end{subequations}
\fi 

\ifnum \value{book}=0
\end{comment}
\fi

\begin{comment}
\section*{Appendix}
The order conditions for the general GARK-ROS scheme~\eqref{eqn:MROS/MROW} up to order three are 
\begin{subequations}
\begin{eqnarray}
\textnormal{order 1:   } && \mathbf{b}^{\{\slow\}\,T} \, \one = 1,  \\
                         && \mathbf{b}^{\{\fast\}\,T} \, \one = 1, \\
\textnormal{order 2:   } &&
\mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\beta}^{\{\slow,\slow\}} \, \boldsymbol{1} = \frac{1}{2}, \\
&&\mathbf{b}^{\{\fast\}\,T} \, \left(
\sum_{\lambda=1}^M \boldsymbol{\beta}^{\{\fast,\fast,\lambda\}} 
\right) \, \boldsymbol{1} = \frac{M}{2}, \\
\textnormal{order 3:   } &&
%\begin{cases}
\mathbf{b}^{\{\slow\}\,T} \, \bigl( (\boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1})\times (\boldsymbol{\alpha}^{\{\slow,\slow\}}\,\mathbf{1}) \bigr) = \frac{1}{3}, \\
&&  \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\beta}^{\{\slow,\slow\}}\, \boldsymbol{\beta}^{\{\slow,\slow\}}\,\mathbf{1} = \frac{1}{6} \\
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\beta}^{\{\slow,\fast,1\}}\, \boldsymbol{\beta}^{\{\fast,\slow,1\}}\,\mathbf{1} = \frac{M}{6} \\
&&
\mathbf{b}^{\{\fast\}\,T} \, \bigl( (\boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1})\times (\boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1} ) 
+ (M-1) 
   \boldsymbol{\alpha}^{\{\fast,\fast\}}\,\mathbf{1}
\bigr) = \frac{3M-1}{6}, \\
&&  \mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M \boldsymbol{\beta}^{\{\fast,\fast,\lambda\}}\, \boldsymbol{\beta}^{\{\fast,\fast,\lambda\}}\,\mathbf{1} = \frac{M}{6} \\
&& \mathbf{b}^{\{\fast\}\,T} \, 
\left( \sum_{\lambda=1}^M \boldsymbol{\beta}^{\{\fast,\slow,\lambda\}}
\right) \, 
 \boldsymbol{\beta}^{\{\slow,\fast,1\}}
 \,\mathbf{1} = \frac{M^2}{6} 
\end{eqnarray}
\end{subequations}
If we couple the slow part with the first step of the fast part only, use the same base schemes for the fast and slow part and choose explicit schemes for the remaining fast steps, the coefficients are given by
\[
\renewcommand{\arraystretch}{1.5}
\begin{array}{c|c}
\A\FF & \A\FS \\ \hline
\A\SF &\A\SS \\ \hline 
{\b}\F  \,\!^T & \b\S  \,\!^T
\end{array} 
%
~~  \raisebox{-10pt}{$\coloneqq$} ~~ 
%
\raisebox{28pt}{$
\begin{array}{cccc|cccc}  
 \sfrac{1}{\mratio} \boldsymbol{\alpha}     &          0                   & \cdots & 0 & \boldsymbol{\alpha}\FSL[1]  \\
 \sfrac{1}{\mratio} \one  \b\FL[1]* &  \sfrac{1}{\mratio} \boldsymbol{\alpha}    & \cdots & 0 &  \boldsymbol{\alpha}\FSL[2]  \\
\vdots                     &                             & \ddots &   & \vdots  \\
 \sfrac{1}{\mratio}\one  \b\FL[1]* &  \sfrac{1}{\mratio}\one  \b\FL[2]*   & \ldots &  \sfrac{1}{\mratio} \boldsymbol{\alpha} &\boldsymbol{\alpha}\FSL[\mratio] \\
\hline 
 \sfrac{1}{\mratio} \boldsymbol{\alpha}\SFL[1] &  0 & \cdots &  0 & \boldsymbol{\alpha}    \\   \hline 
 %
  \sfrac{1}{\mratio} \b\FL[1]* &  \sfrac{1}{\mratio} \b\FL[2]* & \ldots &  \sfrac{1}{\mratio} \b\FL[\mratio]* & \b\S*  
\end{array}
$}\raisebox{-10pt}{,}
\]
%
\[
\renewcommand{\arraystretch}{1.5}
\begin{array}{c|c}
\boldsymbol{G}\FF & \boldsymbol{G}\FS  \\ \hline
\boldsymbol{G}\SF &\boldsymbol{G}\SS 
\end{array} ~~  \coloneqq ~~ 
\raisebox{28pt}{$
\begin{array}{cccc|cccc}  
 \sfrac{1}{\mratio} \boldsymbol{\gamma}      &          0                   & \cdots & 0 & \boldsymbol{\gamma}\FSL[1]  \\
0 &  0        & \cdots & 0 &  0 \\
\vdots                     &                             & \ddots &   & \vdots  \\
 0 & 0   & \ldots &  0 & 0  \\
\hline 
 \sfrac{1}{\mratio} \boldsymbol{\gamma}\SFL[1] &  0 & \cdots &  0 & \boldsymbol{\gamma} 
 \end{array}
 $}.
\]
If we use the explicit and implicit scheme $(\b,\boldsymbol\alpha)$ and $(\b,\boldsymbol\alpha,\boldsymbol\beta)$ of order three given in~\eqref{eq.imim}, the only remaining order conditions are 
\begin{subequations}
\begin{eqnarray}
\textnormal{order 2:   } 
&&\mathbf{b}^{\{\fast\}\,T} \, \left(
\sum_{\lambda=1}^M \boldsymbol{\beta}^{\{\fast,\fast,\lambda\}} 
\right) \, \boldsymbol{1} = \frac{M}{2}, \\
\textnormal{order 3:   } 
&& \mathbf{b}^{\{\slow\}\,T} \, \boldsymbol{\beta}^{\{\slow,\fast,1\}}\, \boldsymbol{\beta}^{\{\fast,\slow,1\}}\,\mathbf{1} = \frac{M}{6} \\
&&  \mathbf{b}^{\{\fast\}\,T} \, \sum_{\lambda=1}^M \boldsymbol{\beta}^{\{\fast,\fast,\lambda\}}\, \boldsymbol{\beta}^{\{\fast,\fast,\lambda\}}\,\mathbf{1} = \frac{M}{6} \\
&& \mathbf{b}^{\{\fast\}\,T} \, 
\left( \sum_{\lambda=1}^M \boldsymbol{\beta}^{\{\fast,\slow,\lambda\}}
\right) \, 
 \boldsymbol{\beta}^{\{\slow,\fast,1\}}
 \,\mathbf{1} = \frac{M^2}{6} 
\end{eqnarray}
\end{subequations}
with $F$ defined in~\eqref{eq.Fl}.
To fulfill the internal consistency conditions, we set the coupling coefficients as 
       \begin{eqnarray*}
    \boldsymbol{\alpha}\FSL[\lambda] & = &
    \sfrac{1}{\mratio} \left( \boldsymbol{\alpha}+ F(\lambda-1) \right), \\
               \boldsymbol{\beta}\FSL[1] & = &
   \sfrac{1}{\mratio} \left( \boldsymbol{\beta}+ 
    \hat \beta \begin{pmatrix}
    0 & 0 & 0 \\ 0 & 0 & 0 \\  -1 & 1  & 0
        \end{pmatrix} 
   \right), \\    
    \boldsymbol{\alpha}\SFL[1] & = &
    \mratio  
    \boldsymbol{\alpha}, \\
    \boldsymbol{\beta}\SFL[1] & = &
    \mratio 
    \left( \boldsymbol{\beta} + \hat \beta 
   \begin{pmatrix}
    0 & 0 & 0 \\ 0 & 0 & 0 \\ -1 & 1  & 0
        \end{pmatrix}   
    \right).
 \end{eqnarray*}
The order conditions now read 
\begin{subequations}
\begin{eqnarray}
\textnormal{order 2:   } 
&&\mathbf{b}^{T} \, \boldsymbol{\gamma} \, \boldsymbol{1} = 0, \\
\textnormal{order 3:   } 
&& \hat \beta  = \frac{M-1}{\beta_{2,1}} \\
&&  (M-1)  \boldsymbol{\alpha} \, \boldsymbol{\alpha} \,\mathbf{1} + {\beta_{2,1}}  \boldsymbol{\beta} \, \boldsymbol{\beta} \,\mathbf{1}= \frac{M}{6} \\
&& \hat \alpha = \frac{3(M+1) \beta_2 - \beta_{2,1} - M}{3 M \beta_{2,1}} 
\end{eqnarray}
The first and third conditions are fulfilled, as both $(\b,\boldsymbol\alpha)$ and $(\b,\boldsymbol\alpha,\boldsymbol\beta)$ are of order three:
\begin{align*}
   \mathbf{b}^{T} \, \boldsymbol{\gamma} \, \boldsymbol{1} & = \mathbf{b}^{T} \, \boldsymbol{\beta} \, \boldsymbol{1} - \mathbf{b}^{T} \, \boldsymbol{\alpha} \, \boldsymbol{1} = \frac{1}{2}-\frac{1}{2}=0, \\
  (M-1)  \boldsymbol{\alpha} \, \boldsymbol{\alpha} \,\mathbf{1} + {\beta_{2,1}}  \boldsymbol{\beta} \, \boldsymbol{\beta} \,\mathbf{1} & = (M-1)  \frac{1}{6} + \frac{1}{6} = \frac{M}{6}.
 \end{align*}
 The other two conditions uniquely fix the remaining parameters $\hat \alpha$ and $\hat \beta$.
 \begin{remark}
 With the choice~\eqref{eq.embed} one gets an embedded scheme of order 2(3). The order 2(3) remains for time-lagged Jacobian, see remark~\ref{remark.time-lagged}.
 \end{remark}

\end{subequations}
\end{comment}



==> packages.tex <==
% A consistent set of packages used throughout the book

%\usepackage[LY1]{fontenc}
%\usepackage[mtbold,LY1]{siammathtime}
\usepackage{epsfig, graphicx}
%\usepackage{epsfig, graphicx, subfigure}
\usepackage{makeidx}
\usepackage{multicol,multirow}
\usepackage{amsmath, amsfonts, amssymb, bbm, bm, mathtools, dsfont}
\usepackage{ulem}
\usepackage{crop}
\usepackage{xcolor,color}
\usepackage{todonotes}
\usepackage{hyperref,url}
% \usepackage{subfig}
\usepackage{caption,subcaption}
%\usepackage[overload]{empheq}
\usepackage{cleveref,scalerel}
\usepackage{xspace,ifthen,mleftright,scalerel}
\usepackage{algorithmic}

\usepackage{tikz}
\usepackage{tikz-qtree}
\usepackage{subfiles}
\usepackage{stmaryrd}
\usepackage{pdflscape}
\usepackage{breqn}
\usepackage{rotating}

\usepackage{array}
\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}  % Vertically-centered & horizontally-centered
\newcolumntype{L}[1]{>{\raggedleft\arraybackslash}m{#1}} % Vertically-centered & horizontally-to-left centered
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}m{#1}} % Vertically-centered & horizontally-to-right

\usepackage{pgfplots}
\pgfplotsset{compat=1.14}
\pgfplotsset{every axis/.append style={
    legend style={at={(0.5,1.05)},anchor=south},
    legend style={/tikz/every even column/.append style={column sep=1cm}},
    legend style={font=\scriptsize},
    legend columns=2
}}

\usepackage{csl}

